When far is better: The Chamberlin-Courant approach to obnoxious committee selection

Classical work on metric space based committee selection problem interprets distance as ``near is better''. In this work, motivated by real-life situations, we interpret distance as ``far is better''. Formally stated, we initiate the study of ``obnoxious'' committee scoring rules when the voters' preferences are expressed via a metric space. To this end, we propose a model where large distances imply high satisfaction and study the egalitarian avatar of the well-known Chamberlin-Courant voting rule and some of its generalizations. For a given integer value $1 \le \lambda \le k$, the committee size k, a voter derives satisfaction from only the $\lambda$-th favorite committee member; the goal is to maximize the satisfaction of the least satisfied voter. For the special case of $\lambda = 1$, this yields the egalitarian Chamberlin-Courant rule. In this paper, we consider general metric space and the special case of a $d$-dimensional Euclidean space. We show that when $\lambda$ is $1$ and $k$, the problem is polynomial-time solvable in $\mathbb{R}^2$ and general metric space, respectively. However, for $\lambda = k-1$, it is NP-hard even in $\mathbb{R}^2$. Thus, we have ``double-dichotomy'' in $\mathbb{R}^2$ with respect to the value of {\lambda}, where the extreme cases are solvable in polynomial time but an intermediate case is NP-hard. Furthermore, this phenomenon appears to be ``tight'' for $\mathbb{R}^2$ because the problem is NP-hard for general metric space, even for $\lambda=1$. Consequently, we are motivated to explore the problem in the realm of (parameterized) approximation algorithms and obtain positive results. Interestingly, we note that this generalization of Chamberlin-Courant rules encodes practical constraints that are relevant to solutions for certain facility locations.

==> algorithm.tex <==



%\section{Algorithm}



\input{algo-polytime}









==> hardness.tex <==


%\section{Lower Bounds}
%In this section we trace the complexity boundary of our problem by giving the promised lower bound results. 
%\subsection{\texorpdfstring{Hardness in General Metrics for $\lambda \ge 1$}{Hardness in General Metrics for lambda ge 1}}
%We present a reduction from {\sc Hitting Set}, defined below, known to be \nph \cite{Karp72} and W$[2]$-parameterized by $k$ \cite{ParamAlgorithms15b}.

%\defproblem{{\sc Hitting Set}}{Set system $(\cU, \cF)$, where $\cU$ is the ground set of $n$ elements, $\cF$ is a family of subsets of $\cU$, and a positive integer $k$}
%{Does there exist $H \subseteq \cU$ of size $k$ such that for any $S \in \cF$, $H \cap S \neq \emptyset$?}

%\noindent{\bf Reduction:} Define a graph $G = (\voters \cup \candidates)$ as follows. For every element $e \in \cU$, we add a candidate $c_e$ to $\candidates$, and for every set $S \in \cF$, we add a voter $v_S$ to $\voters$. $(c_e, v_S)$ is an edge in $G$ iff $e \not\in S$. The weight of all such edges is equal to $1$. Also, for any $c_e, c_e' \in \candidates$, we add an edge of weight $2$. The distance function $d: (\candidates \cup \voters) \to \mathbb{R}^+$ is given by the shortest path distances in $G$. 

\begin{observation} \label{obs:hittingset-equiv}
	For any $e \in \cU$, and $S \in \cF$, $d(c_e, v_S) = 1$ iff $e \not\in S$. Otherwise $d(c_e, v_S) = 3$ iff $e \in S$.
\end{observation}

\begin{lemma} \label{lem:hittingset-equiv}
	$(\cU, \cF)$ admits a hitting set of size $k$ iff there exists a set $H \subseteq \candidates$ of size $k$ such that for any $v_S \in \voters$, $\max_{c_e \in H} d(c_e, v_S) = 3$. 
\end{lemma}
\begin{proof}
	In the forward direction, let $H'' \subseteq \cU$ be a hitting set of size at most $k$. By adding arbitrary elements, we obtain $H' \subseteq \cU$ of size exactly $k$, which remains a hitting set. Let $H$ be the subset of $\candidates$ corresponding to $H'$. Now, for any $S \in \cF$, $H$ contains an element $e$ such that $e \in S$. Thus, for every $v_S \in \voters$, there exists a $c_e \in H$, such that $d(c_e, v_S) = 3$ by Observation \ref{obs:hittingset-equiv}.
	
	In the reverse direction, let $H \subseteq \candidates$ be a set of size $k$ such that for any $v_S \in \voters$,  $\max_{c_e \in H} d(c_e, v_S) = 3$. Let $H'$ be the corresponding subset of elements. 
	For every $v_S \in \cF$, $H$ contains a candidate $c_e$ such that $d(c_e, v_S) = 3$. By Observation \ref{obs:hittingset-equiv}, $e \in S$. This implies that $H'$ is a hitting set.
\end{proof}
This construction shows that it is NP-hard to approximate the problem within a factor of $1/3$. Furthermore, if we reduce from multi-hitting set, where each set needs to be hit at least $\lambda \ge 1$ times for some constant $\lambda$, then it also shows similar results for the $\lambda$-th maximum distance problem. Finally, since the Hitting Set problem is known to be W$[2]$-hard parameterized by the solution size, we also obtain that \problemshort is W$[2]$-hard w.r.t. $k$ in general metrics when $\lambda \ge 1$.

\begin{theorem} \label{thm:apx-hardness}
	For any fixed $1 \le \lambda < k$, \problemshort is \nph. Furthermore, for any fixed $1 \le \lambda < k$, and for any $\alpha \ge 1/3$, \problemshort does not admit a polynomial time $\alpha$-approximation algorithm, unless $\mathsf{P = NP}$. Finally, \problemshort is W$[2]$-hard parameterized by $k$.
\end{theorem}




\input{large-lambda-hardness}



==> introduction-old.tex <==

\section{Introduction}

%Points to cover

%1. Comsoc motivation for voters/candidates in metric space: COI (done)
%2. The mathematical problem resembles clustering type classification/modelling
%2.5 In this context discuss clustering literature-RW
%3. 
%=====================

In an effort to choose a program committee for a conference it is imperative to \hide{select a group of people such} that for all submissions there will be a subset of members with no conflicts of interest (COI).  This type of constraint shows up in large number of applications beyond the above, as we may broaden the notion of COI to include any situation where there is a \Rw{well-understood notion of avoidance.} For example, a situation may demand building large shopping malls as it benefits the local economy but are not necessarily desired by residents living in the vicinity, or at the very least they do not want several malls close to where they live. Thus, the town planners are faced by the challenge of building commercial centers such as malls in viable locations and yet not crowding residential areas with too many of them.  


%could be to find an appropriate menu for a banquet that offers enough options to people with dietary restrictions; choosing a catalogue of films that offers enough diversity of choice for everybody from all age-groups and viewing interests. 

%\Ma{Selection of an awards or research grant approval committee, }

We model this problem in metric spaces where both the potential candidates (e.g. PC members) and voters (i.e conference submissions) are points in the space, and the distance between them quantifies the COI: {\it close is high and far is low}. With this in mind, we frame the question of choosing a PC as that of selecting a $k$-sized subset of {\it candidates} such that for every {\it voter}  there are at least $\lambda$ committee members (i.e {\it representatives}) that are each $t$ distance away.  On the flip side, and often times in literature, close distances are interpreted as desirability and thus a committee whose members are close to all the voters may be desirable in certain situations. In this article, we are studying situations where the goal is to limit ``conflicts'' in an optimal way.   

The framing of the committee selection problem in metric spaces allows us to draw parallels with the clustering problem where the goal is to classify points in terms of distances where close means similar and far means dissimilar. The goal of clustering problems---such as $k$-\textsc{Center} and $k$-\textsc{Median}---is to find groups of similar points, such problems are typically defined as \emph{minimization} problems. In a solution, we assign each point to its nearest \emph{center} (or \emph{candidate}, to stick with the terminology of this paper), and the clusters are obtained by looking at the set of all points that are assigned to a particular center. Observe that all points in a cluster are relatively close to each other, and are thus ``similar''. 

In our context, however, we cannot make the same deduction as two points could be far from a committee member and yet be far from each other. In other words, just because some points\ma{shoudl we stick to voters from here on onwards?} are represented by the same committee members does not mean they themselves have to be close. 

\il{Tanmay, please add some discussions about clustering}

\textbf{Related Work.} 
\td{CS results...}

As mentioned before, most of the clustering---and the closely related Facility Location---problems are posed as minimization problems. However, there are two notable exceptions, namely, the results on OWA proportional voting, and \emph{obnoxious facility}.
\td{paragraph about CS results about OWA $k$-median}
\cite{munagala2021optimal,byrka2017proportional}

The \emph{Obnoxious Facility Location} model is a twist on the standard Facility Location mode. The motivation for this model comes from a similar problem of finding locations for ``undesirable'' facilities, e.g., nuclear reactors or garbage depots, which should be as ``far'' from people as possible. A detailed discussion on the various models considered can be found in the following references \cite{erkut1989analytical,tamir1991obnoxious,kalczynski2022multiple}.

Finally, we mention some similarities of our model with the \emph{fault tolerant} versions of clustering problems, such as $k$-\textsc{Center} or $k$-\textsc{Median} \cite{KumarR13,inamdar2020fault}, also \cite{chakrabarty2017interpolating}. In the latter setting, the clustering objective is defined the distance of a point to its w.r.t.\ $\lambda^{\text{th}}$ closest chosen center, where $\lambda \ge 1$, which is typically assumed to be a small constant. Thus, even if $\lambda -1$ centers chosen in the solution undergo failure, and if they all happen to be nearby a certain point $p$, we still have some (upper) bound on the distance of $p$ to its now-closest center. Note that this motivation of fault tolerance translates naturally into our setting, where we want some (lower) bound on the distance of a voter to its $\lambda^{\text{th}}$ \emph{farthest} candidate, which may be useful of the $\lambda - 1$ farthest \emph{candidates} are unable to perform their duties.

\paragraph{Formal model:} 

\td{copy some stuff from preliminaries...t}


\td{AFter explaining formal model, we discuss specific cases for values of $\lambda$. }




